A GPU-accelerated simulation of rapid intensification of a tropical cyclone with observed heating

This paper presents a limited-area atmospheric simulation of a tropical cyclone accelerated using GPUs. The OpenACC directive-based programming model is used to port the atmospheric model to the GPU. The GPU implementation of the main functions and kernels is discussed. The GPU-accelerated code produces high-fidelity simulations of a realistic tropical cyclone forced by observational latent heating. Performance tests show that the GPU-accelerated code yields energy-efficient simulations and scales well in both the strong and weak limit.

==> sections/Complexity.tex <==
\section{Appendix: Complexity analysis}\label{sec:complexity}

This section presents the complexity of the algorithm in terms of the number of floating-point operations, memory communications, and arithmetic intensity. 

% The MMF version of E3SM model has been ported to GPUs using a directive-based approach \citep{norman2022unprecedented} to achieve strong and weak scaling. 

%------------------------------------------------------%
%   									FLOP
%------------------------------------------------------%
\subsection{Floating-point operations}


We first evaluate the total number of floating-point arithmetic operations, denoted as $F$, throughout the duration of the simulations. The number of operations is evaluated as
\begin{subequations}\label{eq:F1}
\begin{align}
  F &= N^{S}_t N^{S}_e N_p^3 (816 N_p + 4635), \\
\end{align}
\end{subequations}
where $N_t$ is the number of time steps, $N_e$ is the number of elements, and $N_p$ is the number of points in the $x$, $y$, $z$ directions within an element. It is assumed that an element has the same number of points in all directions. In a single simulation, the asymptotic complexity $\mathcal{O}(N_p^4)$ arises from the gradient and divergence kernels, which constitute the dominant cost in constructing the right-rand side vector.

In order to express $F$ in terms of grid size, let us define the number of elements $N_e$ and the number of time steps $N_t$ as follows:
\begin{equation}\label{eq:N_e}
  N_e = \dfrac{L_x L_y L_z}{N^3 \dx \dy \dz},
\end{equation}
where $L_x$, $L_y$, and $L_z$ are the lengths of the domain in the $x$, $y$, $z$ directions, respectively, and $N$ is the order of the basis function.
The number of time steps for the time duration $T$ are counted as
\begin{equation}\label{eq:N_t}
  N_t = \dfrac{T}{\dt}.
\end{equation}

Substituting Eqs.\ \eqref{eq:N_e} and \eqref{eq:N_t} into Eq.~\eqref{eq:F1}, we obtain the following expressions for the number of floating-poing ($F$) operations:
\begin{align}\label{eq:F:final}
  F^S &= \qty(\dfrac{T}{\dt}) \qty(\dfrac{L_x L_y L_z}{N^3\dx \dy \dz}) N_p^3 \qty(816 N_p + 4635).
\end{align}

%------------------------------------------------------%
%   								Communication
%------------------------------------------------------%
\subsection{Communication}\label{sec:communication}

In this analysis, we only consider communications among ranks in the distributed-memory system for comparisons. The transfer of shared data within cores is neglected. The data transfer occurs at the points on the lateral boundaries of the grid partitions in Figure \ref{fig:parallel:decomposition}. The total amount of floating-point numerical data to transfer in bytes ($B$) is evaluated as follows:
\begin{align}\label{eq:B}
  B^S &= N_t^S N_r \qty(784 N_{p,\Gamma}^S),
\end{align}
where $N_r$ is the number of ranks and we assume the use of double precision so that each floating-point number occupies 8 bytes. The number of points at the lateral boundaries of the grid partition $N_{p,\Gamma}$ within a rank is
\begin{align}\label{eq:N_pGamma}
  N_{p,\Gamma}^S &= 2\qty( \dfrac{L_x}{N_{rx}N\dx} + \dfrac{L_y}{N_{ry}N\dy}) \qty(\dfrac{L_z}{N\dz}) N_p^2,\\
\end{align}
where $N_{rx}$ and $N_{ry}$ are the number of ranks in the $x$ and $y$ directions ($N_r=N_{rx}\times N_{ry}$), respectively. Figure \ref{fig:partition} shows the number of elements along each direction at the communicating boundaries. Substituting Eqs.\ \eqref{eq:N_t} and \eqref{eq:N_pGamma} in Eq.~\eqref{eq:B}, we obtain
\begin{align}\label{eq:B:final}
  B^S &= 1568 N_r \qty(\dfrac{T}{\dt}) \qty( \dfrac{L_x}{N_{rx}N\dx} + \dfrac{L_y}{N_{ry}N\dy}) \qty( \dfrac{L_z}{N\dz} )N_p^2.
\end{align}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.4\textwidth]{figures/Figure_partition.png}
  \caption{Dimensions of a grid partition assigned to an MPI rank and the number of elements along each direction. ($N_{ex}$, $N_{ey}$, and $N_{ez}$ are the number of elements along the $x,y,z$ directions.)}\label{fig:partition}
\end{figure}

%------------------------------------------------------%
%   								Arithmetic Intensity
%------------------------------------------------------%
\subsection{Arithmetic intensity}

Arithmetic intensity $I$ is the ratio of total floating-point ($F$) operations to total data movement/bytes ($B$), calculated as $I=F/B$. For simplicity, we assume the following: $N_{rx}=N_{ry}$, $L_x=L_y=L$, $\dx=\dy$, $R_x = R_t = R$ and $R_z=1$. Consequently, the arithmetic intensity for a simulation is calculated using Eqs.\ \eqref{eq:F:final} and \eqref{eq:B:final} as
\begin{align}\label{eq:I}
  I^S &= \dfrac{F^S}{B^S} =  \dfrac{1} { 2\qty( \dfrac{N_{rx}N\dx}{L} ) } N_p (0.520 N_p + 2.956).
\end{align}


==> sections/Numerical_Method.tex <==
\section{Numerical methods}\label{sec:method}

This section describes the numerical methods employed in our limited-area simulations using the standard and MMF approaches. In the MMF, we use the continuous version of the element-based Galerkin method (spectral elements) \citep{giraldo_introduction_2020} to spatially descritize both the LSP and SSP domains. We add the microphysics model to parameterize the SSP models. An implicit sponge layer \citep{klemp2008upper} serves as an upper absorbing boundary condition (ABC). The coupling of the LSP and SSP grids accommodates nonconforming discretization in the vertical direction. Sec.\ \ref{sec:implementation} describes the parallel implementation of our MMF simulations.


==> sections/Results.tex <==

\section{Results}\label{sec:results}

% We test the MMF method on two benchmark problems in numerical weather modeling. In this section, we refer to the simulations without the use of the MMF approach as standard simulations. We assess the performance of the MMF simulation by comparing it with these standard simulations. For the standard simulations, we consider two levels of resolution: a coarse one matching the resolution of the GCM, which is similar to the resolution of the LSP model in the MMF, and a fine one at a much higher resolution for CRM, akin to the resolution of the SSP model in the MMF. We define the grid size as $\Delta x = h/N$, where $h$ is the width of spectral element and $N$ is the order of basis function.

% The simulations were conducted using the 2.0 GHz AMD EPYC 7662 processors on the NPS (Naval Postgraduate School) Supercomputer for parallel runs of the MMF simulation, each element column is assigned to a single processor. As a result, we use 18 cores for the MMF squall line and 216 cores for the MMF supercell case, matching the number of element columns in the LSP domains. 


==> sections/Speedup.tex <==
\subsection{Speedup}

This section presents the results of speedup test for the GPU implementation against the base Fortran code.
